Snapshot Metrics Are Not Enough: Analyzing Software Repositories with Longitudinal Metrics

Software metrics capture information about software development processes and products. These metrics support decision-making, e.g., in team management or dependency selection. However, existing metrics tools measure only a snapshot of a software project. Little attention has been given to enabling engineers to reason about metric trends over time -- longitudinal metrics that give insight about process, not just product. In this work, we present PRiME (PRocess MEtrics), a tool for computing and visualizing process metrics. The currently-supported metrics include productivity, issue density, issue spoilage, and bus factor. We illustrate the value of longitudinal data and conclude with a research agenda. The tool's demo video can be watched at https://youtu.be/YigEHy3_JCo. The source code can be found at https://github.com/SoftwareSystemsLaboratory/prime.

==> archive/parking-lot.tex <==

% GKT: I am keeping this comment here, because it contains our original table, which has now been made more concise.

% \TODO{ ST: Add Citations for each tool and link}
% \TODO{This is one of the contributions of the paper; the analysis and understanding of the state of the art of tools in the space}
% \TODO{A quick summary of this table can be used in this paper}
% \TODO{One of each type of tool in the table}
% \TODO{Describe what each tool type is}
% \center
% \vskip -15pt
% \begin{tabular}{lllllllllllllllllll}
% %   \toprule
%  & \rot{\textbf{Tool Type}} 
%  & \rot{\textbf{Open Source}}                 
%  & \rot{\textbf{Data Warehouse}} 
%  & \rot{\textbf{Chart Generation}} 
%  & \rot{\textbf{Extensible/Modular}}  
%  & \rot{\textbf{Private Repos}}            
%  & \rot{\textbf{Calculate derived Metrics}}  
%  & \rot{\textbf{Continuous Integration Pipeline}}
%  & \rot{\textbf{Process Metrics}}             
%  & \rot{\textbf{Static Code Analysis}} 
%  & \rot{\textbf{Testing Metrics}}      
%  & \rot{\textbf{LOC/KLOC/DLOC}}       
%  & \rot{\textbf{Bus Factor}}                    
%  & \rot{\textbf{Productivity}}          
%  & \rot{\textbf{Issue Density}}
%  & \rot{\textbf{Issue Spoilage}}\\ 
% \toprule
% \textsc{RepoReapers/reaper}\cite{munaiah_curating_2017} & Static Tool &\checkmark & \checkmark & &\checkmark & & \checkmark & & \checkmark & \checkmark & & &  & & & \checkmark & \checkmark & \\ \midrule
% \textsc{ossf/scorecard} & Software Management & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & & \\ \midrule 
% \textsc{ishepard/pydriller}~\cite{spadini_pydriller_2018} & Static Tool &\checkmark & \checkmark & &\checkmark & & \checkmark & & \checkmark & \checkmark & & &  & & & \checkmark & \checkmark & \\ \midrule
% GitHub Insights & Software Management & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & & \\ \midrule 
% NPMS.io & Software Management & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & & & & & & \\ \midrule 
% %Candoia~\cite{candoia} & Platform & \checkmark & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &\checkmark & \checkmark  & & \checkmark & & & & & \\ \midrule
% % TravisTorrent~\cite{travistorr} & Dataset & \checkmark & \checkmark & \checkmark & & & \checkmark &  & & \checkmark & \checkmark & \checkmark & \checkmark & & & & \\ \midrule
% SonarQube & Platform & \checkmark  & \checkmark & \checkmark  & \checkmark  &  & \checkmark & \checkmark & & \checkmark  & \checkmark & \checkmark &\checkmark & &  \\ \midrule
% GoReportCard & Platform & \checkmark  & \checkmark & \checkmark  & \checkmark  &  & \checkmark & \checkmark & & \checkmark  & \checkmark & \checkmark &\checkmark & &  \\ \midrule
% SpotBugs\cite{hovemeyer_finding_2004} & Platform & \checkmark  & \checkmark & \checkmark  & \checkmark  &  & \checkmark & \checkmark & & \checkmark  & \checkmark & \checkmark &\checkmark & &  \\ \midrule \midrule
% % Ares~\cite{ares} & Static Tool & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark & \checkmark & & \checkmark &  & &  & &  & \\ \midrule
% % APEx~\cite{incbl} & Static Tool & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark & \checkmark & & \checkmark &  & \checkmark &  & &  & \\ \midrule
% % RapidRelease~\cite{IMChecker} & Dataset & \checkmark & \checkmark & \checkmark & & & \checkmark & \checkmark & \checkmark & \checkmark & & & & & & & \\ \midrule
% % RepoGrams~\cite{fixme} & Visualizer & \checkmark & \checkmark & & \checkmark & \checkmark & \checkmark & & & \checkmark & \checkmark & & & & & & \\ \bottomrule
% % ConVul~\cite{fixme} & Vulnerability Detector & \checkmark & \checkmark & & & & \checkmark & \checkmark & \checkmark & \checkmark & & & & & & & \\ \midrule
% % EvoME~\cite{fixme} & Software Management & & \checkmark & & & \checkmark & \checkmark & & \checkmark & & \checkmark & \checkmark & \checkmark & & & & \\ \midrule 
% % RepoSkillMiner~\cite{fixme} & Repository Analysis & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & & \checkmark &  & & & & & \checkmark \\ \midrule \midrule
% \name & Tool & \checkmark & \checkmark &   & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark &  &  & \checkmark & \checkmark &\checkmark & \checkmark & \checkmark &\checkmark \\ \bottomrule

% \end{tabular}
% \vskip -10pt
% \label{tab:tools}
% \end{table*}



==> archive/table-related-tools.tex <==
%\TODO{George made this table beautiful again.}
\begin{table*}[ht]
\caption{Representative software metrics tools and their support for longitudinal metrics.}
\center
%\vskip -9pt
\begin{tabular}{ll|ccccccc}
 \textbf{Tool}
 & \textbf{Tool Type}
 & \textbf{Open Source}
%  & \textbf{Process Metrics}
%  & \textbf{Size}
 & \textbf{Bus Factor}
 & \textbf{Productivity}
 & \textbf{Issue Density}
 & \textbf{Spoilage}\\ 
\toprule

RepoReapers/reaper~\cite{munaiah_curating_2017} & Scorecard & \checkmark &  &  &  & \\% \midrule
ossf/scorecard & Scorecard & \checkmark &  &  &  &  \\ \midrule
ishepard/pydriller~\cite{spadini_pydriller_2018} & Framework & \checkmark & & &  & \\% \midrule
Boa~\cite{dyer_boa_2013} & Framework &  &  &  &  & \\ \midrule
GitHub Insights & Dashboard &  &  &  &  & \\% \midrule
GitLab Insights & Dashboard &  &  &  &  & \\ \midrule
npms.io & Platform Monitor & \checkmark &  &  &  & \\% \midrule
GoReportCard & Platform Monitor & \checkmark &  &  &  & \\ \midrule
% SonarQube & Code Reviewer & \checkmark & \checkmark & \checkmark &  &  &  &  & \\ \midrule \midrule
% SpotBugs & IDE Plugin & \checkmark &  &  &  &  &  &  & \\ \midrule \midrule
\name & Process Analyzer & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\bottomrule

\end{tabular}
\vskip -10pt
\label{tab:tools}
\end{table*}


==> authors2.tex <==
\author{
    \IEEEauthorblockN{George K. Thiruvathukal\IEEEauthorrefmark{1}\IEEEauthorrefmark{4}, Cameron Christensen\IEEEauthorrefmark{2}, Xiaoyong Jin\IEEEauthorrefmark{3}, Fran\c{c}ois Tessier\IEEEauthorrefmark{5}\IEEEauthorrefmark{4}, Venkatram Vishwanath\IEEEauthorrefmark{4}}    	
    \IEEEauthorblockA{\IEEEauthorrefmark{1}Loyola University Chicago, Computer Science Department, gkt@cs.luc.edu}
    \IEEEauthorblockA{\IEEEauthorrefmark{2}University of Utah, Scientific Computing and Imaging Institute, cam@sci.utah.edu}
    \IEEEauthorblockA{\IEEEauthorrefmark{3}Argonne National Laboratory, Computational Science Division, xjin@anl.gov}
    \IEEEauthorblockA{\IEEEauthorrefmark{4}Argonne National Laboratory, Leadership Computing Facility, gkt@anl.gov, venkat@anl.gov}
    \IEEEauthorblockA{\IEEEauthorrefmark{5}Swiss National Supercomputing Center, ETH Zurich, Lugano, Switzerland, ftessier@cscs.ch}
}
